Motion-supervised Co-Part Segmentation

Recent co-part segmentation methods mostly operate in a supervised learning setting, which requires a large amount of annotated data for training. To overcome this limitation, we propose a self-supervised deep learning method for co-part segmentation. Differently from previous works, our approach develops the idea that motion information inferred from videos can be leveraged to discover meaningful object parts. To this end, our method relies on pairs of frames sampled from the same video. The network learns to predict part segments together with a representation of the motion between two frames, which permits reconstruction of the target image. Through extensive experimental evaluation on publicly available video sequences we demonstrate that our approach can produce improved segmentation maps with respect to previous self-supervised co-part segmentation approaches.

==> method_old.tex <==
\vspace{-0.2cm}
\section{Method}
In this work, we are interested in training a deep neural network that takes a single image as input and outputs co-part segmentation. Nevertheless, we assume that at training time, we have at disposal a large collection of videos containing objects of the same category. The proposed model is trained using pairs of frames from the same video: $\Xvect_S\in\mathbb{R}^{3\times H\times W}$ and $\Xvect_T\in\mathbb{R}^{3\times H\times W}$ of spatial dimension $H\times W$ and are referred to as \emph{source} and \emph{target} frames, respectively.
%More specifically, the model is trained by reconstructing the target frame $\Tvect$ from the source frame $\Svect$, the estimated segmentation of $\Tvect$, and a sparse motion representation between $\Tvect$ and $\Svect$. 

The overall pipeline is illustrated in Fig.~\ref{fig:pipeline}. Our framework is composed of three main modules. The first module, named \emph{Encoding Module}, is in charge of extracting semantic and motion information from the input frames. We employ a neural network to independently segment the frames $\Xvect_S$ and $\Xvect_T$ into $K\!+\!1$ parts, \ie $K$ segments for the foreground and one for the background. The predicted segments are represented using $K\!+\!1$ channel tensors, \ie $\Yvect_S\in[0,1]^{K+1\times H'\times W'}$ and $\Yvect_T\in[0,1]^{K+1\times H'\times W'}$ associated to the source and the target frames, respectively. Note that, the segmentation source $\Yvect_\textbf{S}$ is predicted independently from the target segmentation and, consequently, the proposed model can be used for still image segmentation at inference time.
 To reduce computations for the segmentation masks we employ a resolution $H'\times W'$, which is smaller than the image resolution. %% Note that the last segmentation part is associated to the background.
We use an U-Net-like architecture with a channel-wise softmax layer at the output to obtain tensors that can be interpreted as part-assignment confidence maps. 


In our self-supervised setting, we also aim at training a generator network that reconstructs the target frame from the source image and the target segmentation. However, reconstructing the target frame directly from its segmentation tends to provide pathological solutions that use $\Yvect_T$ to encode $\Xvect_T$, rather than predicting desired semantic segmentation. In opposition to unsupervised landmark detection, this problem appears particularly in the case of segmentation because of the relatively high dimension of $\Yvect_T$ (typically $64\!\times\!64$). In our case, $\Yvect_T$ is too large a bottleneck and information about the target frame can \emph{leak} to the generator. Therefore, we use the estimated segmentation to reconstruct the target frame in an indirect way. More precisely, we propose to reconstruct the target frame by modeling the motion between the source and the target frames and we include the segmentation $\Yvect_T$ into this motion model. To this end, we introduce a sparse motion representation that describes the motion between the source and the target frames in each segment. The details about our segment motion model are provided in Sec.~\ref{sec:sparse}.


The task of the second module, named \emph{Motion Module}, is to estimate a dense motion field from the sparse motion representation that describes each segment motion.
This dense field $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}\!:\mathbb{R}^2\!\rightarrow\!\mathbb{R}^2$ maps each pixel location in $\Xvect_T$ with its corresponding location in $\Xvect_{S}$. In other words, $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$ is the backward optical flow between the source and the target frames.
%Estimating this dense motion field is the task of the second module of our framework named Dense motion module.
%% We follow a part-based approach to estimate $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$ by modeling the motion within each segment independently. The motion of each segment is described a limited set of parameters to leaking issues.
The estimated motion field comes with an occlusion map $\Ovect_{\mathbf{S} \leftarrow \mathbf{T}} \in \mathbb{R}^{H\times W}$. Occlusion map  indicates frame regions which can be generated by warping the source frame and the occluded areas that need to be inpainted. Details concerning the \textit{Motion Module} are provided in Sec.~\ref{sec:dense}.

Finally, the \emph{Reconstructions Module} reconstructs the target frame from the source frame using an encoder-decoder network. To this aim, we align the intermediate feature representation of the source frame with the pose of the object in the target frame using the estimated dense motion field $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$.
The overall architecture is trained by minimizing a reconstruction loss between the input and reconstructed target frames.
The generation module and the training procedure are described in Sec.~\ref{sec:recTrain}



%% Besides, this encoder network predicts $K$ keypoint locations in $\Xvect_S$ and $\Xvect_T$, along with local descriptors of the object pose (see details in Sec.\ref{sec:sparse}). Importantly, each keypoint is associated with one segmented part. 
%%  

\subsection{Encoding Module}
\label{sec:sparse}
In this section, we detail how we model the motion of each segment. We design our model with the aim of obtaining segments that group together pixels corresponding to object parts that move together. The motion of the pixels within each segment is modeled by an affine transformation. In other words, the dense motion field $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$ can be approximated by an affine transformation on the support corresponding to each segmented part. The encoder network should provide segments such that our affine model is valid. Otherwise, it would lead to wrong dense motion fields $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$ and, subsequently, to high reconstruction loss.

Formally, let $\Yvect_T^k\in[0,1]^{H'\times W'}$ be the $k^{th}$ channel of the segmentation $\Yvect_T$. Even if $\Yvect_T$ and $\Yvect_S$ are tensors with continuous values, for the sake of notation, here we assume that they are binary tensors (this point is further discussed in Sec.~\ref{sec:dense}). We define $\mathcal{Y}_T^k$ as the set of locations associated to the segment $k$, $\mathcal{Y}_T^k=\{z\in[1,H']\times[1,W']~| ~\Yvect_T^k[z]=1\}$. In a similar way, we introduce $\mathcal{Y}_S^k$ for the source segmentation. Assuming that the motion of each segment follows an affine model, this implies that there exists $\Avect\in\mathbb{R}^{2\times 2}$  and $\beta\in\mathbb{R}^{2}$ such that:
\begin{equation}
  \forall z \in\mathcal{Y}_T^k,~\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}(z)
  =  \Avect.z + \beta.  \label{approxaffine}
\end{equation}
In our context, we need to explicitely estimate the affine parameters $\Avect$ and $\beta$ in order to obtain $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$. To this end, we rewrite Eq.~\eqref{approxaffine} as follows: 
\begin{equation}
%%   \medmuskip=0mu
%% \thinmuskip=0mu
  %% \thickmuskip=0mu
  \forall z\in\mathcal{Y}_T^k,~\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}(z)
  =  p_S^k +  \Avect_S^k.{\Avect_T^k}^{-1}\big(z - p_T^k\big)  \label{approxJ}
\end{equation}
where $\Avect_S^k\in\mathbb{R}^{2\times 2}$, ${\Avect_T^k}^{-1}\in\mathbb{R}^{2\times 2}$, $p_S^k\in\mathbb{R}^{2}$ and $p_T^k\in\mathbb{R}^{2}$ are parameters estimated by the encoder network.
This motion decomposition is introduced and formally justified in \cite{siarohin2019neurips}, where it is shown that this decomposition derives from a first order approximation of the motion field $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$. The motivation for this re-writing is to separate terms that are estimated only from the source image (\ie $p_S^k$ and $\Avect_S^k$) from those estimated only from the target (\ie $p_T^k$ and $\Avect_T^k$). 
%% The locations $p_S^k\in\mathbb{R}^{2}$ and $p_T^k\in\mathbb{R}^{2}$ are estimated from the source and from the target frame respectively.
The pixel locations $p_S^k$ and $p_T^k$ can be understood as anchor keypoints associated to the segments $\mathcal{Y}_S^k$ and $\mathcal{Y}_T^k$. Note that, Eq.~\eqref{approxJ} indicates $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}(p_T^k)=p_S^k$ meaning that the pixel value in $\Xvect_T$ at the location $p_T^k\in\mathbb{R}^{2}$ can be obtained by copying the value in $\Xvect_S$ at the location $p_S^k$.
Practically, the anchor keypoints are estimated by the encoder network that outputs $K$ additional channels, one per keypoint.  From each channel, the anchor keypoint location is estimated via \textit{soft-argmax} as in ~\cite{siarohin2018animating,robinson2019laplace,siarohin2019neurips}. 

By introducing the matrices $\Avect_S^k$ and ${\Avect_T^k}$, the motion within $\mathcal{Y}_T^k$ of  $p_T^k\in\mathbb{R}^{2}$ is modeled by an affine transformation, thus accounting for transformations that cannot be obtained by simple pixel-shift.
%% Concerning the matrix $J_k$,  we employ the parametrization introduced in \cite{siarohin2019neurips}. $J_k$ is decomposed as follows:
%% \begin{equation}
%%     \label{eq:Ak}
%%      \Jvect^k=\Avect_S^k.{\Avect_T^k}^{-1}.
%% \end{equation}
The matrices $\Avect_S^k\in\mathbb{R}^{2\times 2}$ and $\Avect_T^k\in\mathbb{R}^{2\times 2}$ are independently estimated from the source and the target frames, respectively. Practically, each $\Avect^k$ is computed by the encoder network with four additional outputs. From these 4-channel tensors, we obtain the coefficients of the matrices $A_S^k$ and $A_T^k$ by computing spatial weighted average using as weights the confidence map of the corresponding keypoint as in \cite{siarohin2019neurips}.
In the end, the encoder outputs a total of $6K\!+\!1$ channels: $K\!+\!1$ for the segmentation, $K$ for the anchor keypoints and $4K$ for the $\Avect^k$ matrices. 


%% The aim of the second module is to twofold. First, the module outputs an estimator $\hat{\Tvect}_{\mathbf{S} \leftarrow \mathbf{T}}\in \mathbb{R}^{2\times H'\times W'}$ of the dense motion field $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$. This estimator is later used to reconstruct $\Xvect_T$ from $\Xvect_S$ in the generation module. Second, it outputs an occlusion map indicating to the generation module which frame regions should be inpainted.


\subsection{Motion Module}
\label{sec:dense}
We now detail how the dense motion fields $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$ is obtained by combining the segment motion representations and the predicted segmentation.
For each segment, we employ the model given by Eq.~\eqref{approxJ} to obtain $K$ motion fields $\Tvect^k\in \mathbb{R}^{2\times H'\times W'}$ of $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$, valid in each respective segment  $\mathcal{Y}_T^k$. The tensor $\Tvect^k$ can be interpreted as the optical flow for the pixels of the segment $\mathcal{Y}_T^k$ between the source and target frames. Note that the last motion field $\Tvect^{K+1}$ is associated to the background. We assuming a static background and consequently set $\Tvect^{K+1}=z$. We consider that each object part corresponds to a segment in $\Yvect_T$ and that its motion can be encoded by its corresponding segment motion descriptor. Consequently, we obtain the following discretized estimator $\hat{\Tvect}_{\mathbf{S} \leftarrow \mathbf{T}}$ of the motion field $\mathcal{T}_{\mathbf{S} \leftarrow \mathbf{T}}$:
\begin{equation}
\hat{\Tvect}_{\mathbf{S} \leftarrow \mathbf{T}}=\sum_{k=1}^{K+1} \Yvect_T^{k}\otimes \Tvect^{k} \label{eq:estim}
\end{equation}
where $\otimes$ denotes the element-wise product. In Eq.~\eqref{eq:estim}, the segmentation mask $\Yvect_T^{k}$ is used to assign a motion field $\Tvect^{k}$ to each location. In other words, the encoder network must output segmentation masks that allows the dense motion module to correctly assign a motion field $\Tvect^{k}$ to each location $z$. The segmentation mask must gather together locations that move in the same way.
In practice, $\Yvect_T^{k}$ are continous tensors. Consequently, Eq.~\eqref{eq:estim} can be interpreted as a soft assignment model that selects the appropriate motion vector for each pixel location. The use of continous tensors facilitates gradient-based optimization. 


\paragraph{Occlusion.}
The motion module also outputs an occlusion map $\Ovect_{\mathbf{S} \leftarrow \mathbf{T}} \in [0,1]^{H'\times W'}$. It indicates what pixels can be obtained by warping the source frame and the ones that must be inpainted. Modeling occlusions enforce better background/foreground separation since poor segmentation maps would lead to poor occlusion maps and this would affect the final reconstruction quality. $\Ovect_{\mathbf{S} \leftarrow \mathbf{T}}$ is computed from the source and target segmentations. 

We estimate the foreground locations in the source frame by merging the K object parts $\Fvect_S\!=\!\sum_{k=1}^K\Yvect_S^k$. Occluded locations are then defined as locations corresponding to the background in the target ($\Yvect_T^{K+1}\!=\!1$) but to the foreground in the source frame.  Formally, the occlusion map is given by: 
\begin{equation}
\Ovect_{\mathbf{S} \leftarrow \mathbf{T}}= (\Yvect_T^{K+1}\otimes\Fvect_S)
\end{equation}


An alternative approach could consist in using an additional network in order to predict occlusion masks from the source image and the segmentation motion similarly to \cite{siarohin2019neurips}. However this approach would suffer from a major issue. Indeed, occlusion is mostly used for reducing parts of the background wrongly classified as the foreground, which is later referred as a \emph{false fg}. A large \emph{false fg} in the source frame implies a significant amount of information useful for background reconstruction. Consequently, reconstruction loss minimization would lead to predicted occlusion mask with an important amount of \emph{false fg}.\steph{Not clear why our approach does not suffer from this }

Note that, simply providing occlusion to the generator would be problematic since information about the target frame would \emph{leak} through $\Yvect_T^{K+1}$. To this end, we prevent the gradient flow trough the $\Yvect_T^{K+1}$, by detaching $\Yvect_T^{K+1}$ from the computational graph.



\subsection{Reconstruction and Training}
\label{sec:recTrain}

In this section, we describe how we make use of the estimated dense motion field to reconstruct the target frame. Then, we provide the details of our training procedure.
We employ a generator network $G$ that reconstructs the target frame by warping the source frame features according to the computed dense motion. $G$ has an encoder-decoder architecture with a deformation layer in its bottleneck. This deformation layer takes as input a feature map $\xivect\in\mathbb{R}^{C\times H'\times W'}$, the estimated dense motion $\hat{\Tvect}_{\mathbf{S} \leftarrow \mathbf{T}}\in\mathbb{R}^{2\times H'\times W'}$ and the occlusion map ${\Ovect}_{\mathbf{S} \leftarrow \mathbf{T}}$. We use ${\Ovect}_{\mathbf{S} \leftarrow \mathbf{T}}$ to mask out the feature map locations that should be inpainted. Thus, the occlusion mask lowers the impact of the features located in the occluded parts. The deformation layer output is defined as follows:
\begin{equation}
\xivect'=(1-\Ovect_{\mathbf{S} \leftarrow \mathbf{T}})\odot \mathcal{W}(\xivect,\hat{\Tvect}_{\mathbf{S} \leftarrow \mathbf{T}})\label{eq:wrap}
\end{equation}
where $\mathcal{W}(\cdot,\cdot)$ denotes the back-warping operation and $\odot$ denotes the Hadamard product.
The warping operation is implemented in a differentiable manner using the bilinear sampler of Jaderberg~\etal\cite{jaderberg2015spatial}. 

\begin{table*}[t]
    \centering
    \def\arraystretch{0.9}
    \begin{tabular}{lcccc}
         \rotatebox{90}{\hspace{0.45cm}\emph{Naive}} & \includegraphics[width=0.12\columnwidth]{figures/taichi/naive/taichi-170-overlay-naive.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/naive/taichi-170-hard-naive.png} & \includegraphics[width=0.12\columnwidth]{figures/taichi/naive/taichi-174-overlay-naive.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/naive/taichi-174-hard-naive.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/naive/vox-8-overlay-naive.png}\includegraphics[width=0.12\columnwidth]{figures/vox/naive/vox-8-hard-naive.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/naive/vox-4-overlay-naive.png}\includegraphics[width=0.12\columnwidth]{figures/vox/naive/vox-4-hard-naive.png} \\
         
         \rotatebox{90}{\hspace{0.25cm}\emph{Shift-only}} & \includegraphics[width=0.12\columnwidth]{figures/taichi/kp-only/taichi-170-overlay-kp.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/kp-only/taichi-170-hard-kp.png} & \includegraphics[width=0.12\columnwidth]{figures/taichi/kp-only/taichi-174-overlay-kp.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/kp-only/taichi-174-hard-kp.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/kp-only/vox-8-overlay-kp.png}\includegraphics[width=0.12\columnwidth]{figures/vox/kp-only/vox-8-hard-kp.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/kp-only/vox-4-overlay-kp.png}\includegraphics[width=0.12\columnwidth]{figures/vox/kp-only/vox-4-hard-kp.png} \\
         
         \rotatebox{90}{\hspace{0.25cm}\emph{Affine-only}} & \includegraphics[width=0.12\columnwidth]{figures/taichi/no-occlusion/taichi-170-overlay-no-occlusion.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/no-occlusion/taichi-170-hard-no-occlusion.png} & \includegraphics[width=0.12\columnwidth]{figures/taichi/no-occlusion/taichi-174-overlay-no-occlusion.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/no-occlusion/taichi-174-hard-no-occlusion.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/no-occlusion/vox-8-overlay-no-occlusion.png}\includegraphics[width=0.12\columnwidth]{figures/vox/no-occlusion/vox-8-hard-no-occlusion.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/no-occlusion/vox-4-overlay-no-occlusion.png}\includegraphics[width=0.12\columnwidth]{figures/vox/no-occlusion/vox-4-hard-no-occlusion.png} \\
         
         \rotatebox{90}{\hspace{0cm}\emph{$\Ovect$-back-prop}} & \includegraphics[width=0.12\columnwidth]{figures/taichi/occlusion-attached/taichi-170-overlay-occlusion-attached.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/occlusion-attached/taichi-170-hard-occlusion-attached.png} & \includegraphics[width=0.12\columnwidth]{figures/taichi/occlusion-attached/taichi-174-overlay-occlusion-attached.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/occlusion-attached/taichi-174-hard-occlusion-attached.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/occlusion-attached/vox-8-overlay-occlusion-attached.png}\includegraphics[width=0.12\columnwidth]{figures/vox/occlusion-attached/vox-8-hard-occlusion-attached.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/occlusion-attached/vox-4-overlay-occlusion-attached.png}\includegraphics[width=0.12\columnwidth]{figures/vox/occlusion-attached/vox-4-hard-occlusion-attached.png} \\
         
         %\rotatebox{90}{\emph{$\Ovect$-detached}} & \includegraphics[width=0.12\columnwidth]{figures/taichi/occlusion-detached/taichi-170-overlay-occlusion-detached.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/occlusion-detached/taichi-170-hard-occlusion-detached.png} & \includegraphics[width=0.12\columnwidth]{figures/taichi/occlusion-detached/taichi-174-overlay-occlusion-detached.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/occlusion-detached/taichi-174-hard-occlusion-detached.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/occlusion-detached/vox-8-overlay-occlusion-detached.png}\includegraphics[width=0.12\columnwidth]{figures/vox/occlusion-detached/vox-8-hard-occlusion-detached.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/occlusion-detached/vox-4-overlay-occlusion-detached.png}\includegraphics[width=0.12\columnwidth]{figures/vox/occlusion-detached/vox-4-hard-occlusion-detached.png} \\
         
         \rotatebox{90}{\hspace{0.6cm}\emph{Full}} & \includegraphics[width=0.12\columnwidth]{figures/taichi/full/taichi-170-overlay-monkey.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/full/taichi-170-hard-monkey.png} & \includegraphics[width=0.12\columnwidth]{figures/taichi/full/taichi-174-overlay-monkey.png}\includegraphics[width=0.12\columnwidth]{figures/taichi/full/taichi-174-hard-monkey.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/full/vox-8-overlay-monkey.png}\includegraphics[width=0.12\columnwidth]{figures/vox/full/vox-8-hard-monkey.png} & \includegraphics[width=0.12\columnwidth]{figures/vox/full/vox-4-overlay-monkey.png}\includegraphics[width=0.12\columnwidth]{figures/vox/full/vox-4-hard-monkey.png} \\
    \end{tabular}

    \captionof{figure}{\textbf{Visual comparison of our method and baselines}. In the even columns segmentation mask is depicted, while in the odd columns original image with overlayed segmentation is shown. Columns one through four corresponds to \emph{Tai-Chi-HD} dataset, and columns five through  eight show \emph{VoxCeleb} dataset.}
    \label{fig:ablations}

\end{table*}{}

\paragraph{Training Losses.}
We train our model in an end-to-end fashion.
The reconstruction loss used is our main driving loss. It is based on the perceptual loss of Johnson \etal~\cite{johnson2016perceptual} and uses a pre-trained VGG-19~\cite{DBLP:journals/corr/SimonyanZ14a} network to asses reconstruction quality. 
%\alex{We use the following 5 layers: conv1\_2, conv2\_2, conv3\_2, conv4\_2,
%conv5\_2, similarly to~\cite{wang2018video}.}\steph{If it is the same than 35 I would not list these layers since the notations are not clear.}\sergey{agree with Steph, we can move them to supplement}
Given the input target frame $\Xvect_T$ and its corresponding reconstructed frame $\bar{\Xvect_T}$, the reconstruction loss is defined as:
  \begin{equation}
    \mathcal{L}_{rec}(\bar{\Xvect_T}, \Xvect_T)  = \sum_{i=1}^{I} \left|\Phi_i(\bar{\Xvect_T}) - \Phi_i(\Xvect_T) \right|,
\end{equation}
where $\Phi_i(\cdot)$ denotes the $i^{th}$ channel feature extracted from a specific VGG-19~\cite{DBLP:journals/corr/SimonyanZ14a} layer and $I$ denotes the number of feature channels in this layer. In addition, this loss is computed at several resolutions, similarly to MS-SSIM~\cite{wang2003multiscale,tang2018dual}.  

%% \alex{This loss we don't use}
Furthermore, following previous unsupervised keypoint detection methods~\cite{jakabunsupervised,Zhang_2018_CVPR} we employ an equivariance loss to force the network to predict segment motion representations that are consistent with respect to known geometric transformations. As in~\cite{siarohin2019neurips}, we impose an equivariance loss with respect to anchor keypoints $p^k$ and matrices $\Avect^k$, we refer to this loss as  $\mathcal{L}_{eq}$.
Finally, the overall loss function is:
\begin{equation}
\mathcal{L}_{tot}=\mathcal{L}_{rec}+\mathcal{L}_{eq}.
  \end{equation}
  
  \eli{We need the formula for equivariance}
  
  
\eli{\textbf{Difference with [33]}. We would like to clarify the key differences with [33]. 
%First, from an applicative point of view, our model directly predict a segmentation from an input frame.%, while [33] does not. 
 while [33] can not. Indeed, [33] requires at least 2 frames to predict a keypoint neighbourhoods, even during the inference. This makes predictions of [33] highly dependent on the other frame in a pair. For e.g., we observe that: (i) if there is not enough motion between 2 frames then [33] will not predict any neighbourhoods; (ii) [33] may include a lot of background motion in the prediction. Since our model makes independent predictions it always encodes semantically meaningful parts.
%Indeed, [33] can be used estimate the key-point neibourhoods which can serve as segmentation. However this requires at least 2 frames, and these neighbourhoods would be different from pair to pair also neighbourhoods could focus on some parts which are not relevant to semantics. For example, we observe that [33] include a lot of background motion in the prediction, which in turn make this model inefficient for segmentation
%cannot predict segmentation from a single image. [33]
%requires two frames to predict keypoint neighbourhoods that are used only to specify the support of their piecewise-affine motion model.
%This neighbourhoods can be thought as segmentations
%Since these neighbourhoods are based on motion between frames, it may focus on some parts which are not relevant to semantics. For example, we observe that [33] include a lot of background motion in the prediction, which in turn make this model inefficient for segmentation. %Second, the first order model of [33] uses segmentation only to specify the support of their piecewise-affine motion model. Conversely, in our model, segmentation maks are predicted independently from each image by the encoder network. 
%This difference in the segmentation prediction leads to different flow fields.
}

% Assuming an image $\vect{X}$ and its anchor keypoints $p\!=\!\{p^k\}_{k=1..K}$, we sample a random spatial deformation $\mathcal{D}$ and estimate the keypoints $\tilde{p}\!=\!\{\tilde{p}^{k}\}_{k=1..K}$ of $\mathcal{D}(\Xvect)$. We define the equivariance loss as follows:
% \begin{equation}
% \mathcal{L}(p,\tilde{p})= \sum_{k=1}^K ||p^k-\tilde{p}^k||^2.
%   \end{equation}
% Besides, we also impose an equivariance loss on the $\Avect_k$ matrices used in our affine model. More specifically, we employ the equivariance loss of \cite{siarohin2019neurips}. The total of the two equivariance losses is referred to as $\mathcal{L}_{eq}$ \eli{formula???}. 




